Fast Geometric Projections for Local Robustness Certification

Local robustness ensures that a model classifies all inputs within an $\ell_2$-ball consistently, which precludes various forms of adversarial inputs. In this paper, we present a fast procedure for checking local robustness in feed-forward neural networks with piecewise-linear activation functions. Such networks partition the input space into a set of convex polyhedral regions in which the network's behavior is linear; hence, a systematic search for decision boundaries within the regions around a given input is sufficient for assessing robustness. Crucially, we show how the regions around a point can be analyzed using simple geometric projections, thus admitting an efficient, highly-parallel GPU implementation that excels particularly for the $\ell_2$ norm, where previous work has been less effective. Empirically we find this approach to be far more precise than many approximate verification approaches, while at the same time performing multiple orders of magnitude faster than complete verifiers, and scaling to much deeper networks.

==> figures/table_linf_large.tex <==
% !TEX root=../paper.tex

\begin{tabular}{l|ccccc|cccc|cccc}
\toprule
\multicolumn{1}{c}{} &
% \multicolumn{3}{c}{TreeFGP} &
\multicolumn{5}{c}{FGP} & 
\multicolumn{4}{c}{ERAN} & 
\multicolumn{4}{c}{GeoCert} \\

Model & 
Time (s) & \rob & \norob & \unk & \timeout &
Time (s) & \rob & \norob & \timeout &
Time (s) & \rob & \norob & \timeout \\ \midrule

mnist20x3 & 
	& & & & & 
	0.229 & 59 & 41 & 0 &
	 & & &  \\
mnist20x6 & 
	 & & & & &
	 0.814 & 56 & 44 & 0 &
	 & & & \\
mnist20x9 & 
	 & & & & &
	 11.109 & 51 & 40 & 9 &
	 & & & \\
mnist40x3 & 
	 & & & & &
	 1.661 & 64 & 35 & 1 &
	 & & & \\
mnist60x3 & 
	 & & & & &
	 30.752 & 54 & 29 & 17 &
	 & & & \\ \midrule \midrule


fmnist100x6* &
	 & & & & &
	 4.445 & 15 & 84 & 1 &
	 & & & \\
fmnist100x10* &
	 & & & & &
	 7.943 & 18 & 70 & 12 &
	 & & & \\
mnist-cnn16.32.100* &
	 & & & & &
	 & & & &
	 & & & \\
\bottomrule
\end{tabular}%


==> future.tex <==
%\todo{AF: This should likely be merged with the conclusion or the related work. Probably related work}

Several possible improvements to our implementation are left as future work.
% The algorithm presented in Section \ref{sec:algorithm} is norm-independent, but its performance relies on efficiently computing projections using a GPU.
% We implemented this for the $\ell_2$ and $\ell_\infty$ norms;
% extending our approach to other norms would require similar techniques, which already exist for the $\ell_1$ norm~\cite{l1projections, Higherl1projections} for instance.
E.g., As our implementation runs mostly on a GPU, we should be able to more aggressively fall back on parallel executions of LP solvers, which run on CPUs, when our analysis is inconclusive. %is activation regions.
% Finally, we plan to add support for convolutional neural networks.

%\begin{itemize}
%
%\item Extend to other norms
%\item Efficient parallelism
%\item Heuristics to check high-risk regions first \todo{If not implemented by the deadline}
%\item Extension to CNNs
%
%\end{itemize}


==> heuristics.tex <==
% !TEX root=./paper.tex

% In this section, we present different heuristics that we implement to both speed up our analysis and
% reduce the number of \unknown returned by our algorithm.

\subsection{Improving the Completeness of the Algorithm}\label{sec:heur:compl}

The vanilla version of our algorithm presented in Section~\ref{sec:algorithm} stops and possibly
returns \unknown at the first decision boundary encountered. 
We now present two heuristics to reduce the number of \unknown results returned, at the price of increased complexity.
These heuristics are disabled by default in our implementation.
We leave it to the user to enable them when deemed necessary.

\paragraph{Exploring the Full Queue}
If the analysis of a decision boundary is inconclusive, Algorithm~\ref{alg:naive}, as presented so far, stops and returns \unknown.
We implement a variant of Algorithm~\ref{alg:naive} where we instead record the presence of an ambiguous decision boundary but continue exploring other regions in the queue.
If we entirely empty the queue after unsuccessfully analyzing a decision boundary, we nevertheless return \unknown.
However, oftentimes a true adversarial example is found during the continued search, allowing us to return \notrobust conclusively.

The correctness of our algorithm still holds in this variant:
an inconclusive analysis of a decision boundary leads to either returning \unknown, or exhibiting a true adversarial example found subsequently.

\paragraph{Falling Back on LP Solving}
Existing complete tools \cite{katz17reluplex,katz19marabou,ProvableBallFitting,tjeng18MIP,Fischetti18MILP,Cheng17Resilience} often rely heavily on solvers to analyze models. 
When we cannot rule out adversarial examples in a specific activation region, we can query an LP solver, since both the activation constraints delimiting a region and the decision boundaries inside this region are linear constraints.
This allows us to efficiently discharge many verification conditions through fast geometric projections while providing a complete, but slower, variant of our algorithm.

\subsection{Speeding up the Analysis}\label{sec:heur:speed}

In Section~\ref{sec:algorithm}, Algorithm~\ref{alg:naive} is presented at a high level without regard to performance.
In this section, we give an overview of the key optimizations we include in our implementation of \algname that are independent of the high-level behavior of the algorithm.
% The correctness of Algorithm~\ref{alg:naive} is independent of how we iterate over the queue of constraints to analyze.
% In this section, we present different iteration strategies to search the regions that might have a higher
% chance of containing adversarial examples first.

\paragraph{Analyzing Decision Boundaries First}
The correctness of Algorithm~\ref{alg:naive} is independent of how we iterate over the queue of constraints to analyze.
As such, we can prioritize the most relevant constraints, i.e. decision boundaries.
Note, however, that this optimization cannot be used when searching for a certified lower bound (Algorithm~\ref{alg:lowerbounds}) as it would break the correctness of the algorithm.

% Compared to more complex priority queues, both enqueuing and dequeuing elements remains constant-time.

% \paragraph{Checking higher risk regions first}
% \todo{If implemented, write this}

\paragraph{Batching}
Most deep learning software is designed to easily enable efficient batch computations on a GPU.
In particular, the gradient backpropagations for computing constraints (Section~\ref{sec:impl:boundaries}) and the dot product projections for calculating distances (Section~\ref{sec:impl:distances}) lend themselves well to batching on the GPU.
We leverage this in our implementation of \algname by dequeuing multiple elements from the queue at once and calculating the constraints and constraint distances for the corresponding regions in parallel.
We find that this optimization enables a speedup of up to 2x on large examples for a well-chosen batch size ($\sim$10-100).



==> impact.tex <==
This paper provides a new technique for network verification.
With the widespread adoption of machine learning from areas ranging from collision
avoidance systems to autonomous cars, adversarial examples in networks can lead to
bugs and attacks with dramatic consequences.

Through this work, we address this issue in different ways.
First, our framework allows us to provide formal guarantees about the robustness of many points
in a network.
Second, our framework can be used to conclude that an input might be adversarial, and thus
should not be trusted or accepted.

Although network verification is still a recent research area that does not yet enable verification
of large, widely-used networks such as ResNet, this paper proposes an approach scaling to
deeper, more realistic networks than previous work.
Therefore, we believe it to be an important step towards proving strong security guarantees
of existing systems relying on machine learning.


==> implementation.tex <==
% !TEX root=./paper.tex

In this section, we describe the key insights that allow us to implement Algorithm~\ref{alg:naive} efficiently, and describe various optimizations we employ to improve its practicality.
In Sections~\ref{sec:impl:boundaries} and \ref{sec:impl:distances} we elaborate on the insights and implementation details relevant to computing constraints and approximating their distance from $x$.
Section~\ref{sec:heur:compl} describes heuristics for reducing the number of \unknown results \algname returns, and Section~\ref{sec:heur:speed} presents optimizations we implement that speed up our analysis.

\subsection{Computing Activation Region Boundaries}\label{sec:impl:boundaries}

Recall that an activation constraint, $C_u$, which is satisied when $\modelfn_u(x) \geq 0 \Longleftrightarrow \ap(u)$,
is a linear constraint with coefficients $w_u$, and intercepts, $b_u$.
The computation of these weights and intercepts does not depend on a particular point in $\ar$ --- only on the activation pattern, $\ap$.
Thus, \emph{we can compute the boundaries of an activation region, $\ar$, knowing only the corresponding activation pattern, $\ap$}.

In practice, the coefficients, $w_u$, correspond to the gradient of $\modelfn_u$ with respect to its inputs, evaluated at a point in $\ar$.
However, frameworks that perform automatic differentiation typically require a concrete point for evaluation of the gradient.
Thus, we compute the gradient via backpropagation with the activation vectors, $a_i$, where the position in $a_i$ corresponding
to neuron, $u$, takes value 1 if $\ap(u)$ is $true$ and 0 otherwise.
The intercepts, $b_u$, are computed via a forward computation using the activation vectors, with $x$ set to 0.
These operations can easily be implemented to run efficiently on a GPU.

\paragraph{Decision Boundaries}
For a sigmoid network, there is at most a single decision boundary within any given activation region, which can be computed via gradient backpropagation as discussed above.
In the case of a softmax model with multiple classes, we have an output for each class.
A decision boundary for a point, $x$, given class, $i$, states that $f(x)_i \geq f(x)_j$, for $j \neq i$.
Thus, for models with $n$ classes, the decision boundary consists of $n-1$ linear constraints derived from the difference of the model's output at the selected class and the model's output at each of the other classes.


\subsection{Distances to Constraints}\label{sec:impl:distances}

We observe that when working with the $\ell_2$ norm, we can efficiently compute projections using the dot product (we add that projections can be computed efficiently for other norms as well, e.g., the $\ell_\infty$ norm; see Section~\ref{sec:eval:linf}).
This computation can be trivially performed on many constraints in parallel by a GPU.

The distance from $x$ to its projection onto a hyperplane constraint, $C$, gives a \emph{lower bound} on the distance from $x$ to the part of $C$ that is feasible when the other constraints are taken into con{}sideration.
This allows us to soundly determine if a boundary constraint is further than $\epsilon$ from $x$, implying local robustness, and is substantially faster than using constraint solving to discover the true distance.
In our evaluation, we find that in high dimensions, the projected distance is an accurate enough lower bound to make \algname practical.

% Explanation of how to actually collect constraints, compute projections, different tricks used to implement the algorithm

% Python/Keras.

% Most of the algorithm can be batched and run on GPU.

% LP Solving not on GPU, but using (TBD) library.

% (To Be Counted) LoCs




==> proof.tex <==
% !TEX root=./paper.tex

%\todo{come up with different term rather than ``partial''} correctness of our algorithm:
We show that when \algname returns \notrobust, there exists an adversarial example, and when it returns \robust, the model is locally robust at $x$, with radius $\epsilon$. However, the algorithm may also return \unknown, in which case we do not claim anything about the robustness of the model. A complete proof of Theorem~\ref{thm:correctness} is provided in the supplementary material.

\begin{theorem}\label{thm:correctness}
(1) When \algname returns \notrobust, there exists an adversarial example, $p$, such that $\norm{x - p} \leq \epsilon$ and $\modelclass(x) \neq \modelclass(p)$. 
(2) When \algname returns \robust, Equation~\ref{eq:local-robustness} holds.
\end{theorem}



\subsection{Certified Lower Bounds}
\label{sect:lower-bound}

%\todo{AF: Move this at the end of section 2, and provide a snippet of the modified algorithm + give an intuition regarding why this is correct}
%\todo{Bryan: Agreed, but adjust the description of the queue, since at that point, you haven't said that it's two queues internally}
We now consider the related problem of finding a \emph{lower bound} on the local robustness of the network.
A variant of Algorithm~\ref{alg:naive}, given by Algorithm~\ref{alg:lowerbounds}, can provide certified lower bounds by using a priority queue.
In this variant, constraints are enqueued with a priority corresponding to their distance from $x$, such that the closest constraint to $x$ is always at the front of the queue.
We keep track of the current certified lower bound in a variable, $\beta$. 
At each iteration, we set $\beta$ to the maximum of the old $\beta$ and the distance from $x$ to the constraint at the front of the queue.

The algorithm terminates either when all constraints at distance less than the  initially specified $\epsilon$ were handled,
or when a decision boundary for which the initial algorithm returns \unknown or \notrobust is found. 
In the first case, we return $\epsilon$; in the second, we return the value stored in $\beta$ at this iteration.

The proof of this variant is similar to the proof of Algorithm~\ref{alg:naive}.
It relies on the following loop invariant:

\begin{loopinvariant}\label{thm:loopinvariant}
% At each iteration 
(1) all activation regions at distance less than $\beta$ from $x$ were previously visited, (2) $\beta$ is always smaller than $\epsilon$,
and (3) there is no adversarial point at distance less than $\beta$.
\end{loopinvariant}

%\begin{proof}
%Loop Invariant~\ref{thm:loopinvariant} trivially holds on entry of the loop since $bound$ is initialized to 0.
%Proving that the invariant is maintained is more interesting. 
%Suppose that $bound$ increases to $bound'$. 
%It must then be shown that there is no unvisited activation region at distance less than $bound'$.
%We proceed again by contradiction:
%assume there was such a region, $\ar$, containing a point, $p$, such that $\norm{x - p} \leq bound'$.
%Again, let us consider the segment from $x$ to $p$, and the path, $P$, it induces.
%Let us consider $\ar_i$, the first region of $P$ at distance greater than $bound$ that was not previously visited.
%If no such region exists, then $\ar$ is at distance less than $bound$ from $x$, and so by our induction hypothesis, it was already visited.
%% and therefore visited since the queue is a priority queue and $bound < bound'$.
%otherwise, $\ar_{i-1}$ was visited, and the activation constraint, $C$, between $\ar_{i-1}$ and $\ar_i$ is such that $d(x, C) \leq bound' \leq \epsilon$.
%Therefore, $C$ (which leads to $\ar_i$) was already added to the queue with priority less than $bound'$, and by virtue of the priority queue, it was explored before the current iteration, which yields a contradiction.
%
%If $bound$ does not increase, the invariant still trivially holds.
%This case can happen because our computation of the distance to constraints is an underapproximation of the true distance to the feasible portion of the constraint, as is illustrated in Figure~\ref{fig:boundconstraint}.
%\end{proof}
%
%
%\begin{figure}
%\centering
%\includegraphics[page=1, width=.85\columnwidth]{figures/boundconstraint_small}
%\caption{Illustration of a constraint, $C$, whose projection-based distance, $d$, is smaller than the true distance, $d'$, from $x$ to the feasible portion of $C$ in the shaded activation region.
%}
%\label{fig:boundconstraint}
%\end{figure}


==> proof_tree.tex <==
% !TEX root = paper.tex

% \subsection{Leveraging the Compositional Structure of Feed-forward Networks}

We build upon the proof of Theorem~\ref{thm:correctness} presented in Appendix~\ref{sec:fgp_proof}
To prove the correctness of our tree-based exploration, we only need to prove that the additional regions we filter out either are unreachable, or are explored through a different path.

To prove this assertion, we consider the case where we are exploring a region $\bar{A}$,
reached from a previously explored region $\bar{A}_{prev}$ by flipping a neuron $u$ at layer $N$. 
Let us assume that our optimization filters out a region $\bar{A}_{next}$ reachable from $\bar{A}$ by flipping a neuron $u'$.
This means that $u'$ belongs to an earlier layer.

As the corresponding activation patterns $A$ and $A_{prev}$ only differ in $u$,
all the constraints corresponding to neurons in earlier layers are the same for $\bar{A}$ and $\bar{A}_{prev}$.
In particular, this means that the activation constraint associated to $u'$ is the same in both regions.
Hence, $\bar{A'}$, where $A'$ is $A_{prev}$ with $u'$ flipped, is added to the queue of regions to explore. 
Now, $A'$ and $A_{next}$ only differ in the neuron $u$, and $u$ is at a later layer than $u'$.
Thus, if $\bar{A}_{next}$ is in the $\epsilon$-ball, it will be reached from $\bar{A'}$

It might be the case that $u'$ itself is filtered out in $\bar{A}_{prev}$. The intuition here is that we can then go "one step up" in the path
of regions leading from the initial region to $\bar{A}$ and apply a similar argument. 
Similarly to the proof of Theorem~\ref{thm:correctness}, this can be formalized by an induction on the length of the paths of explored regions.

